Hypergraph Vision Transformers: Images are More than Nodes, More than Edges

Recent advancements in computer vision have highlighted the scalability of Vision Transformers (ViTs) across various tasks, yet challenges remain in balancing adaptability, computational efficiency, and the ability to model higher-order relationships. Vision Graph Neural Networks (ViGs) offer an alternative by leveraging graph-based methodologies but are hindered by the computational bottlenecks of clustering algorithms used for edge generation. To address these issues, we propose the Hypergraph Vision Transformer (HgVT), which incorporates a hierarchical bipartite hypergraph structure into the vision transformer framework to capture higher-order semantic relationships while maintaining computational efficiency. HgVT leverages population and diversity regularization for dynamic hypergraph construction without clustering, and expert edge pooling to enhance semantic extraction and facilitate graph-based image retrieval. Empirical results demonstrate that HgVT achieves strong performance on image classification and retrieval, positioning it as an efficient framework for semantic-based vision tasks.

==> Figures/evaluation/ablation_table_v1.tex <==
\begin{table}[ht]
    \caption{ImageNet-100 \cite{tian2020contrastive} ablations for the HgVT-TL model. The top two rows contain default configurations for comparison. The \Yes and \No symbols represent that the method is or is not used. Numbers for non-boolean, and pooling methods: Average~(\BlackNum{A}), Image~(\BlackNum{I}), Expert~(\BlackNum{E}), Average+Image~(\BlackNum{BA}), and Expert+Image~(\BlackNum{BE}).}
    \centering
    \vspace{0.5em}
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{c| c | p{0.1cm} p{0.1cm} p{0.1cm} c| p{0.1cm} p{0.1cm} p{0.1cm} p{0.1cm} p{0.1cm} p{0.1cm} c |c c| c c}
        % First row with multicolumn spanning for "Accuracy"
        % Second row with individual column names
        Ablation on $\downarrow$ & 
        % data augmentation
        \rhead{Repeats} &
        % regularization
        \rhead{Dropout} &
        \rhead{Stoch. Decay} &
        \rhead{Diversity} &
        \rhead{Population} &
        %\rhead{SAM} &
        % architecture 
        \rhead{CNN Stem} &
        \rhead{$\mathbf{X}_\adj = \mathbf{X}$} &
        \rhead{Tied QKV} &
        \rhead{Tied FFN} &
        %\rhead{$d$ Multiplier} &
        \rhead{Vertex MHSA} &
        \rhead{Pooling Op} & 
        \rhead{Layers} & 
        % accuarcy
        \rhead{top-1 Acc.} & 
        \rhead{top-5 Acc.} &
        % stats
        \rhead{Params (M)} &
        \rhead{FLOPS (G)}
        \\\toprule
        % defaults
        %CMC \cite{tian2020contrastive} & 
        %-- & -- & -- & -- & -- & -- & -- & -- & -- &  -- & -- & -- & 
        % accuracy
        %81.5 & -- & 12 & 0.26 \vspace{-1em} \\ 
        HgVT-TL (baseline) 
        % 4 repeats, dropout 0.1, stoch decay, diversity, population, cnn_stem
        & \BlackNum{2} & \Yes & \Yes & \Yes & \Yes & \Yes & 
        % split adj, split KQV, split FFN, VSA, 10 layers, ave pooling
        \No & \No & \No & \Yes & \BlackNum{A} &  \BlackNum{10} &
        * & * \\
        \hline
        % data augmentation
        \multirow{2}{*}{Data aug.} 
        % 1 repeats, dropout 0.1, stoch decay, diversity, population, cnn_stem
        & \BlackNum{1} & \yes & \yes & \yes & \yes & \yes & 
        % split adj, split KQV, split FFN, VSA,  ave pooling, 10 layers
        \no & \no & \no & \yes  & \GrayNum{A} &  \GrayNum{10} &
        * & * \\
        % 3 repeats, dropout 0.1, stoch decay, diversity, population, cnn_stem
        & \BlackNum{3} & \yes & \yes & \yes & \yes & \yes & 
        % split adj, split KQV, split FFN, VSA, ave pooling, 10 layers
        \no & \no & \no & \yes & \GrayNum{A} &  \GrayNum{10} &
        * & * \\
% Omit this case since 3 performed worse than 2
%        % 4 repeats, dropout 0.1, stoch decay, diversity, population, cnn_stem
%        & \BlackNum{4} & \yes & \yes & \yes & \yes & \yes & 
%        % split adj, split KQV, split FFN, VSA, ave pooling, 10 layers
%        \no & \no & \no & \yes & \GrayNum{A} &  \GrayNum{10} &
%        * & * \\
        \hline
        % Regularization
        \multirow{2}{*}{Regularization} 
        % 2 repeats, no dropout, stoch decay, diversity, population, cnn_stem
        & \GrayNum{2} & \No & \yes & \yes & \yes & \yes & 
        % split adj, split KQV, split FFN,VSA,  ave pooling, 10 layers
        \no & \no & \no & \yes & \GrayNum{A} &  \GrayNum{10} &
        * & * \\
        % 2 repeats, dropout, no stoch decay, diversity, population, cnn_stem
        & \GrayNum{2} & \yes & \No & \yes & \yes & \yes & 
        % split adj, split KQV, split FFN, VSA,  ave pooling, 10 layers
        \no & \no & \no & \yes  & \GrayNum{A} &  \GrayNum{10} &
        * & * \\   
        % 2 repeats, dropout, stoch decay, no diversity, population, cnn_stem
        & \GrayNum{2} & \yes & \yes & \No & \yes & \yes & 
        % split adj, split KQV, split FFN, VSA,  ave pooling, 10 layers
        \no & \no & \no & \yes  & \GrayNum{A} &  \GrayNum{10} &
        * & * \\   
        % 2 repeats, dropout, stoch decay, diversity, no population, cnn_stem
        & \GrayNum{2} & \yes & \yes & \yes & \No & \yes & 
        % split adj, split KQV, split FFN, VSA,  ave pooling, 10 layers
        \no & \no & \no & \yes &  \GrayNum{A} &  \GrayNum{10} &
        * & * \\   
        \hline
        % Architecture
        \multirow{2}{*}{Architecture} 
        % 2 repeats, dropout, stoch decay, diversity, population, no cnn_stem
        & \GrayNum{2} & \yes & \yes & \yes & \yes & \No & 
        % split adj, split KQV, split FFN, VSA,  ave pooling, 10 layers
        \no & \no & \no & \GrayNum{1} &  \GrayNum{A} &  \GrayNum{10} &
        * & * \\  
        % 2 repeats, dropout, stoch decay, diversity, population, no cnn_stem
        & \GrayNum{2} & \yes & \yes & \yes & \yes & \yes & 
        % split adj, split KQV, split FFN, no VSA,  ave pooling, 10 layers
        \no & \no & \no & \No &  \GrayNum{A} &  \GrayNum{10} &
        * & * \\  
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        & * & \BlackNum{3} & \GrayNum{2}  \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> Figures/evaluation/ablation_table_v2.tex <==
\begin{table}[h!]
    \caption{ImageNet-100 ablations with HgVT-Lt. Indicating used~(\Yes) or not used~(\No), and pooling methods: Average~(\BlackNum{A}), Image~(\BlackNum{I}), Expert~(\BlackNum{E}), Average+Image~(\BlackNum{AI}), and Expert+Image~(\BlackNum{EI}).
    } \label{tab:ablations}
    \centering
    \vspace{-0.5em}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c| p{0.1cm} p{0.1cm} p{0.1cm} c| 
    p{0.1cm} p{0.1cm} p{0.2cm} c |
    p{0.6cm} p{0.4cm} c | p{0.4cm} c}
        % First row with multicolumn spanning for "Accuracy"
        % Second row with individual column names
        Ablation on $\downarrow$ & 
        % regularization
        \rhead{CLS Dropout} &
        \rhead{Stoch. Decay} &
        \rhead{Diversity} &
        \rhead{Population} &
        %\rhead{SAM} &
        % architecture 
        \rhead{Tied FFN} &
        \rhead{$\mathbf{X}_\adj = \mathbf{X}$} &
        \rhead{$d_f$ Mult.} &
        %\rhead{$d$ Multiplier} &
        \rhead{Pooling Op} & 
        % metrics
        \hspace{0.1cm}
        \rhead{Top-1 Acc.} & 
        \hspace{0.01cm}
        \rhead{Edge Entropy} &
        \rhead{Silhouette} &
        % stats
        \hspace{0.02cm}
        \rhead{Params (M)} &
        \rhead{FLOPs (G)}
        \\\toprule
        % defaults
        %CMC \cite{tian2020contrastive} & 
        %-- & -- & -- & -- & -- & -- & -- & -- & -- &  -- & -- & -- & 
        % accuracy
        %81.5 & -- & 12 & 0.26 \vspace{-1em} \\ 
        none: HgVT-Lt
        % dropout 0.1, stoch decay, diversity, population |
        & \No & \Yes & \Yes & \Yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \Yes & \Yes & \BlackNum{1} & \BlackNum{E} &
        % top-1, HE, SIL | Params FLOPs
        82.52 &  3.13 & 0.749 &  6.62 & 0.88\\
        \hline
        % Regularization
        \multirow{5}{*}{Regularization} 

        
        % using class dropout
        % dropout 0.1, stoch decay, diversity, population |
        & \Yes & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        82.23 &  3.13 & 0.751 &  6.62 & 0.88 \\
       

        % no stochastic decay
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \No & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        81.89 &  3.12 & 0.745 &  6.62 & 0.88 \\

        % no diversity
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \No & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        80.79 &  1.99 & 0.723 &  6.62 & 0.88 \\

        % no population
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \No & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        81.79 &  3.89 & 0.639 &  6.62 & 0.88 \\
        

        % no diversity or population
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \No & \No & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        81.99 &  3.58 & 0.610 &  6.62 & 0.88 \\
        
        \hline
        % Architecture
        \multirow{4}{*}{Architecture} 

        % split FFN, split adj
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \No & \yes & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        82.89 &  3.09 & 0.741 &  9.86 & 0.87 \\

        % split ffn, tied adj
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \No & \No & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        78.62 &  2.27 & 0.808 &  5.84 & 0.56  \\

        % tied ffn, tied adj
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \No & \GrayNum{1} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        76.95 &  2.12 & 0.780 &  4.40 & 0.56  \\

        % tied ffn, tied adj, 1.5 mult
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \No & \BlackNum{1.5} & \GrayNum{E} &
        % top-1, HE, SIL | Params FLOPs
        77.46 &  2.05 & 0.770 &  9.62 & 1.18 \\

        \hline
        \multirow{4}{*}{Pooling} 

        % mean
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \BlackNum{A} &
        % top-1, HE, SIL | Params FLOPs
        82.06 &  3.07 & 0.747 &  6.62 & 0.88 \\

        % image
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \BlackNum{I} &
        % top-1, HE, SIL | Params FLOPs
        84.08 &  2.93 & 0.760 &  6.62 & 0.88 \\

        % bothA
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \BlackNum{AI} &
        % top-1, HE, SIL | Params FLOPs
        84.24 &  3.08 & 0.736 &  6.75 & 0.88 \\

        % bothE
        % dropout 0.1, stoch decay, diversity, population |
        & \no & \yes & \yes & \yes & 
        % Tied FFN, split adj, d mult, expert pooling |
        \yes & \yes & \GrayNum{1} & \BlackNum{EI} &
        % top-1, HE, SIL | Params FLOPs
        84.32 &  2.94 & 0.741 &  6.75 & 0.88 \\
        
        \bottomrule
    \end{tabular}
    }
\end{table}

==> Figures/evaluation/imnet_retrieval.tex <==
\begin{table}[h!]
    \caption{Image Retrieval on \mbox{ImageNet-1k} with proposed search methods:~PS, APS, VS, and AVS. Reporting Top-1 accuracy, mAP@10~(\%), and 1-NN-CLIP-L hit-rate@10~(\%). 
    } \label{tab:imnet_ret}
    \centering
    \vspace{-0.5em}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l | c | c | c c | c c }
    \toprule
    Model & Top-1 & Metric & PS & APS & VS & AVS \\
    \midrule
    MRL-128 \cite{Kusupati2022MatryoshkaRL} & 70.52 & mAP@10 & 64.94 & 65.20 & -- & -- \\
     MRL-256 \cite{Kusupati2022MatryoshkaRL} & 70.62 & mAP@10 & 65.04 & 65.20 & -- & -- \\
MRL-512 \cite{Kusupati2022MatryoshkaRL} & 70.82 & mAP@10 & 65.14 & 65.20 & -- & -- \\
     MRL-1024 \cite{Kusupati2022MatryoshkaRL} & 70.89 & mAP@10 & 65.16 & 65.20 & -- & -- \\
     \midrule
%HgVT-Lt (ours) & -- & mAP@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
HgVT-Ti (ours) & 76.18 & mAP@10 & 73.26 & 12.34 & 73.01 & 12.34 \\
%HgVT-S (ours) & 12.34 & mAP@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
%HgVT-B (ours) & 12.34 & mAP@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
%     \midrule 
%HgVT-Lt (ours) & -- & 1NN-hit@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
HgVT-Ti (ours) & 76.18 & 1NN-hit@10 & 25.47 & 12.34 & 25.21 & 12.34 \\
%HgVT-S (ours) & 12.34 & 1NN-hit@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
%HgVT-B (ours) & 12.34 & 1NN-hit@10 & 12.34 & 12.34 & 12.34 & 12.34 \\
     
    \bottomrule
    \end{tabular}
    }
\end{table}

==> Figures/evaluation/imnet_sota.tex <==
\begin{table}[h!]
    \caption{\mbox{ImageNet-1k} results for HgVT and other isotropic networks. \CNN CNN, \Transformer Transformer, 
    %\MLP MLP, 
    \GNN GNN, \HGNN HGNN, and \HGVT HgVT.
    }\label{tab:short_sota}
    \vspace{-0.5em}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
        \toprule
        \textbf{Model} & \textbf{Resolution}  & \textbf{Params} & \textbf{FLOPs} & \textbf{Top-1} & \textbf{Top-5} \\
        \midrule
        % ConvNets
        \CNN ResMLP-S12 conv3x3 \cite{res_mpl_paper} 
                                & 224x224 & 16.7M & 3.2B & 77.0 & -- \\
        \CNN ConvMixer-768/32 \cite{convmixer} 
                                & 224x224 & 21.1M & 20.9B & 80.2 & -- \\
        \CNN ConvMixer-1536/20 \cite{convmixer} 
                                & 224x224 & 51.6M & 51.1B & 81.4 & -- \\
        \midrule
        % Transformers
        \Transformer ViT-B/16 \cite{vit16x16words} 
                                & 384x384 & 86.4M & 55.5B & 77.9 & -- \\
        \Transformer DeiT-Ti  \cite{deit_paper}
                                & 224x224 & 5.7M & 1.3B & 72.2 & 91.1 \\
        \Transformer DeiT-S  \cite{deit_paper}
                                & 224x224 & 22.1M & 4.6B & 79.8 & 95.0 \\
        \Transformer DeiT-B  \cite{deit_paper}
                                & 224x224 & 86.4M & 17.6B & 81.8 & 95.7 \\
        \midrule
        % ViGs
        \GNN ViG-Ti \cite{vig_paper}
                                & 224x224 & 7.1M & 1.3B & 73.9 & 92.0 \\
        \GNN ViG-S \cite{vig_paper}
                                & 224x224 & 22.7M & 4.5B & 80.4 & 95.2 \\
        \GNN ViG-B \cite{vig_paper}
                                & 224x224 & 86.8M & 17.7B & 82.3 & 95.9 \\
        \midrule
        % ViHGNN
        \HGNN ViHGNN-Ti \cite{vihgnn_paper}
                                & 224x224 & 8.2M & 1.8B & 74.3 & 92.5 \\
        \HGNN ViHGNN-S \cite{vihgnn_paper}
                                & 224x224 & 23.2M & 5.6B & 81.5 & 95.7 \\
        \HGNN ViHGNN-B \cite{vihgnn_paper}
                                & 224x224 & 88.1M & 19.4B & 82.9 & 96.2 \\
        \midrule
        % HgVT
        \HGVT HgVT-Ti (ours) & 224x224 & -- & -- & -- & -- \\
        \HGVT HgVT-S (ours) & 224x224 & -- & -- & -- & -- \\
        \HGVT HgVT-B (ours) & 224x224 & -- & -- & -- & -- \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> Figures/evaluation/repeat_table.tex <==
\begin{table}[ht]
    \caption{Comparing Top-1 impact of repeating the last block of HgVT-Lt on ImageNet-100 \cite{tian2020contrastive}, keeping total FLOPs constant. }\label{tab:repeats}
    \centering
    \resizebox{0.42\textwidth}{!}{
    \begin{tabular}{l|c c c c}
        \toprule
        $L$ + N Repeats $\rightarrow$ & $12+0$ & $11+1$ & $10+2$ & $9+3$ \\
        \midrule
        Top-1      & 12.34 & 12.34 & 12.34 & 12.34  \\
        Params (M) & 12.34 & 12.34 & 12.34 & 12.34 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> sections/method.tex <==
\section{A Hypergraph Vision Transformer}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{Figures/method/arch_diagram.png}
  \caption{HgVT Architecture Diagram, composed of stacked HgVT blocks with adjacency matrix $\mathbf{A}$, vertex features $\mathbf{X}^\V$, and hyperedge features $\mathbf{X}^\E$. Edge attention flow is shown with gray arrows. Pooling is only applied to the subset $\mathbf{X}^{(:vE)}$; input norms and residual adds are omitted for clarity. }
  \label{fig:hgvt_arch}
\end{figure}

The Hypergraph Vision Transformer (HgVT) adapts the architecture of standard Vision Transformers by incorporating hypergraph features to enhance image analysis capabilities. 
Similar to Vision Transformers, HgVT utilizes a patch embedding layer as its entry point, followed by an isotropic stack of $L$ HgVT blocks, each based on the ubiquitous Llama blocks\footnote{HgVT uses fixed sinusoidal position embeddings rather than rotary position embeddings.}
\cite{touvron2023llama}, culminating in feature pooling and a classifier head. 
Configured to process both vertex and edge information, the blocks include six main components: adjacency mask computation, vertex self-attention, edge aggregate attention, edge distribution attention, and separate feed-forward networks for vertices and edges. 
This configuration facilitates dynamic bipartite graph construction within each block, allowing the model to adaptively refine the input image's representative hypergraph.


Four key feature matrices -- $\mathbf{X}^\V$, $\mathbf{X}^\V_\adj$, $\mathbf{X}^\E$, and $\mathbf{X}^\E_\adj$ -- represent the bipartite hypergraph features and are progressively updated in each HgVT block in an interleaved manner. 
Each block also constructs a new adjacency matrix $\mathbf{A}$ from the input $\mathbf{X}^\V_\adj$ and $\mathbf{X}^\E_\adj$ matricies, which then contributes to the attention layers within that block. 
As illustrated in Figure \ref{fig:hgvt_arch}, this approach allows for the dynamic integration and processing of these matrices within each HgVT block, facilitating effective feature interaction and updating.

For succinct discussion in subsequent sections, the update process for each layer $l$ is encapsulated using the following compact notation:

\vspace{-1em}
\begin{equation}
\textstyle 
\mathbf{X}^{(*, l+1)}_* = \mathbf{X}^{(*, l)}_* + \mathbf{X}^{(*, l)\prime}_*, \quad \mathbf{X}^{(*, l)\prime}_* = f\left(\mathrm{RN}\left(\mathbf{X}^{(*, l)}_*\right), \dots, \mathbf{A}^{(l)}\right)
\end{equation}
\vspace{-1em}

where $\mathrm{RN}(\cdot)$ denotes the RMS Norm \cite{zhang2019root}, and $\mathbf{X}^{(*, l)}_*$ includes both vertex features and hyperedge features, along with their respective adjacency features. The update function $f(\cdot)$ can utilize all four normalized feature matrices and the adjacency matrix $\mathbf{A}^{(l)}$, which is updated once per HgVT block.


\subsection{Dynamic Adjacency Formation}

Dynamically establishing the hypergraph structure is crucial for adaptability across varying semantic and spatial structures inherent in different image inputs.
Mirroring the query-key interactions found in attention mechanisms, HgVT utilizes cosine similarity to evaluate the alignment between vertex and hyperedge adjacency features.
This similarity assessment allows hyperedges to effectively 'query' vertices for relevant features, establishing a scale-invariant comparison that focuses on the directionality of embedding vectors. 
To convert the cosine similarity to adjacency membership, we then form the soft adjacency matrix $\mathbf{A}$ with a sharpened sigmoid function, detailed as follows:
\begin{equation}
    \mathbf{A} = \sigma\left(\alpha \cdot \mathbf{\tilde{X}}^\V_\adj \left[\mathbf{\tilde{X}}^\E_\adj\right]^T\right), \;\;\; \mathbf{\tilde{X}}^{(*)}_\adj = \frac{\mathbf{X}^{(*)}_\adj}{||\mathbf{X}^{(*)}_\adj||_2 + \epsilon}
\end{equation}
% tensor arithmetic form
%\begin{equation}
%    A_i^j = \sigma\left(\alpha \cdot \tilde{X}^{\V,a}_{\adj, i} \tilde{X}^{\E,j}_{\adj, a}\right)
%\end{equation}
where \(\mathbf{\tilde{X}}^{(*)}_\adj\) represents the L2-normalized adjacency feature matrix.
Here, $\sigma$ denotes the sigmoid function, and $\alpha=4$ acts as a sharpening factor, enhancing the sigmoid's effectiveness by pushing intermediate values toward the extremes.
The hard membership adjacency matrix \(\mathbf{\hat{A}} = [\mathbf{A} > 0.5]\) transforms these sigmoid outputs into binary memberships, crucial for defining significant hypergraph relationships and suitable for sparse attention masking.
In configurations where feature matrices and adjacency feature matrices are tied ($\mathbf{X}^{(*)}_\adj = \mathbf{X}^{(*)}$), $\mathbf{X}^{(*)}_\adj$ is computed as $\mathbf{X}^{(*)} \mathbf{W}_*$, using a learned projection matrix to adapt features for adjacency computation and maintain embedding adaptability.

%, since the range of the sigmoid function is bounded between 0 and 1. In configurations with tied feature and adjacency feature matrices , learned projection matrices are used to create a pseudo adjacency query.

% \subsection{\red{HgVT Blocks: Hyperedges as Communication Pools}}
% \red{Simplify the architecture information and move the details to the appendix}
% \red{Focus on the high level idea of graph construction, and breaking up the message passing scheme into V->V, V->E, and E->V}.


\subsection{Vertex Message Passing with Sparse Self-Attention}

Shifting from traditional hypergraph models, which typically employ a gather $\rightarrow$ scatter mechanism for processing vertex-hyperedge interactions, HgVT reconceptualizes hyperedges as communication pools that facilitate dynamic and efficient information flow among vertices and their associated hyperedges.
Instead of relying on a single dense attention operation, HgVT organizes communication into two distinct streams: intra-hyperedge message passing and interactions between hyperedges  and their constituent vertices. 
By enabling direct message passing within hyperedges, the model significantly enhances inter-vertex communication, allowing for more nuanced integration of contextual information.
Furthermore, this configuration restricts interactions to vertices that share hyperedges, naturally inducing sparsity in the interaction matrix and substantially reducing computational overhead. 
The strategy for message passing between vertices within a hyperedge ($\mathcal{V}_e\rightarrow \mathcal{V}_e$) is implemented through the following update process:
% \begin{equation}
%     \mathbf{X}^{\V\prime} = \mathrm{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^T}{\sqrt{d_k}} + \mathbf{B}\right) \mathbf{V},\;\;\;\; \mathbf{Y}=\mathbf{X}^\V \mathbf{W}_Y,\; Y\in\{Q,K,V\}
% \end{equation}

% \begin{equation}
%     \mathbf{X}^{\V\prime} = \mathrm{softmax}\left(\frac{\left(\mathbf{X}^{\V}\mathbf{W}_Q\right)\left(\mathbf{X}^{\V}\mathbf{W}_K\right)^T}{\sqrt{d_k}} + \mathbf{B}\right)\left(\mathbf{X}^{\V}\mathbf{W}_V\right)
% \end{equation}
\vspace{-1em}
\begin{equation}
\textstyle 
    \mathbf{X}^{\V\prime} = \mathrm{softmax}\left(\left(\mathbf{X}^{\V}\mathbf{W}_Q\right)\left(\mathbf{X}^{\V}\mathbf{W}_K\right)^T + \mathbf{B}\right)\left(\mathbf{X}^{\V}\mathbf{W}_V\right),\;\; \mathbf{B} = 1 -\left[\left(\mathbf{\hat{A}}\mathbf{\hat{A}}^T\right) > 0 \right]
\end{equation}
% \begin{equation}
%     \mathbf{X}^{\V\prime} = \mathrm{softmax}\left(d_k^{-\frac{1}{2}}\left(\mathbf{X}^{\V}\mathbf{W}_Q\right)\left(\mathbf{X}^{\V}\mathbf{W}_K\right)^T + \mathbf{B}\right)\left(\mathbf{X}^{\V}\mathbf{W}_V\right)
% \end{equation}
In this equation, the mask $\mathbf{B}\in\{0,1\}^{|V|\times|V|}$ is a dynamically computed nased on the connectivity within the hyperedges, derived from the hard adjacency matrix $\hat{\mathbf{A}}\in\{0,1\}^{|V|\times|E|}$.
This masking ensures that attention computations are confined to vertices within the same hyperedge, enhancing communication efficiency. 
Additionally, for simplification, the typical attention scaling factor $1/\sqrt{d_k}$, which is generally used to stabilize the softmax calculations, is omitted from the above equation.


% \begin{equation}
%     \textstyle 
%     \mathbf{B} = 1 -\left[\left(\mathbf{\hat{A}}\mathbf{\hat{A}}^T\right) > 0 \right]
% \end{equation}

% tensor arithmetic form
%\begin{equation}
%    B_i^j = 1 - \left[\left(\hat{A}_i^k \hat{A}_k^j\right) > 0 \right] 
%\end{equation}





% tensor arithmetic form
%\begin{equation}
%    H^{\N,b,\prime}_i = \mathrm{softmax}_j\left(\frac{Q_i^a K_a^j}{\sqrt{d_k}} + B_i^j\right)V_j^b, \;\;\; Y_i^a = H^{\N,c}_i W_{Y,c}^a,\;\; Y\in\{Q,K,V\}
%\end{equation}

\subsection{Hyperedge Message Passing with Fuzzy Cross-Attention}

Completing the concept of hyperedges as dynamic communication pools outlined in the previous section, HgVT utilizes cross-attention mechanisms to facilitate interactions between hyperedges and their constituent vertices.
These mechanisms -- hyperedge aggregation attention ($\mathcal{V}_e\rightarrow \mathcal{E}_e$), focusing on gathering information, and hyperedge distribution attention ($\mathcal{E}_e\rightarrow \mathcal{V}_e$), dedicated to scattering information -- leverages HgVT's unique bipartite representation for effective management of information flows within these pools.
By modulating the attention logits with the soft adjacency matrix~$\mathbf{A}$ via a Hadamard product, the model introduces a layer of ``fuzziness'' to the typical cross-attention mechanism.
Such modulation dynamically aligns the model’s response to the varied connectivity patterns typical in hypergraph structures, thereby enhancing both precision and adaptability in processing information.
The equations that formalize these attention processes are presented below:
% \begin{equation}
%      \textstyle 
%     \mathbf{X}^{\E\prime} = \mathrm{softmax}\left(\left(\mathbf{X}^{\E}\mathbf{W}_Q\right)\left(\mathbf{X}^{\V}\mathbf{W}_K\right)^T\circ \mathbf{A}^T + \mathbf{M}^T\right)\left(\mathbf{X}^{\V}\mathbf{W}_V\right)
% \end{equation}
\begin{eqnarray}
    \textstyle
    \mathbf{X}^{\E\prime} &=& \mathrm{softmax}\left(\left(\mathbf{X}^{\E}\mathbf{W}_Q\right)\left(\mathbf{X}^{\V}\mathbf{W}_K\right)^T\circ \mathbf{A}^T + \mathbf{M}^T\right)\left(\mathbf{X}^{\V}\mathbf{W}_V\right)  \\
     \mathbf{X}^{\V\prime} &=& \mathrm{softmax}\left(\left(\mathbf{X}^{\V}\mathbf{W}_Q\right)\left(\mathbf{X}^{\E}\mathbf{W}_K\right)^T\circ \mathbf{A} + \mathbf{M}\right)\left(\mathbf{X}^{\E}\mathbf{W}_V\right)   
\end{eqnarray}
In this framework, the soft adjacency matrix $\mathbf{A}\in\mathbb{R}^{|V|\times|E|}$ modulates the attention logits through a Hadamard product ($\circ$), dynamically reflecting the true connectivity of vertices to hyperedges and providing a gradient path to update the weights used to compute the adjacency feature matrices.
Concurrently, the static interaction mask $\mathbf{M}\in\{0,1\}^{|V|\times|E|}$ prevents virtual hyperedges ($v\mathcal{E}$) from interacting with image vertices ($i\mathcal{V}$), ensuring the maintenance of the hierarchical hypergraph structure described in Section \ref{sec:imposing_hierarchical_structure} within the architecture.
As before, the $1/\sqrt{d_k}$ factor is omitted for clarity.

% tensor arithmetic form
%\begin{eqnarray}
%    H^{\E,b,\prime}_i &=& \mathrm{softmax}_j\left(\frac{Q_i^a K_a^j A_i^j}{\sqrt{d_k}} + M_i^j\right)V_j^b \nonumber\\
%    Q_i^a &=& H^{\E,c}_i W_{Q,c}^a, \;\;\;\; Y_i^a = H^{\N,c}_i W_{Y,c}^a,\;\; Y\in\{K,V\}
%\end{eqnarray}

% \begin{equation}
%      \textstyle 
%     \mathbf{X}^{\V\prime} = \mathrm{softmax}\left(\left(\mathbf{X}^{\V}\mathbf{W}_Q\right)\left(\mathbf{X}^{\E}\mathbf{W}_K\right)^T\circ \mathbf{A} + \mathbf{M}\right)\left(\mathbf{X}^{\E}\mathbf{W}_V\right)
% \end{equation}

% tensor arithmetic form
%\begin{eqnarray}
%    H^{\E,b,\prime}_i &=& \mathrm{softmax}_j\left(\frac{Q_i^a K_a^j A_i^j}{\sqrt{d_k}} + M_i^j\right)V_j^b \nonumber\\
%    Q_i^a &=& H^{\N,c}_i W_{Q,c}^a, \;\;\;\; Y_i^a = H^{\E,c}_i W_{Y,c}^a,\;\; Y\in\{K,V\}
%\end{eqnarray}

\subsection{Hypergraph Feature Processing}

Distinct point-wise feed-forward networks (FFNs) are utilized to process vertex and hyperedge features independently within the HgVT blocks, ensuring differentiated processing for each set within the bipartite representation.
These features are integrated with adjacency features through a dense, fully-connected mechanism, allowing the FFN to effectively combine both immediate and relational attributes.
By updating both feature types and their adjacency embeddings within the same FFN layer, the model centralizes computational tasks and simplifies the message passing process by focusing solely on feature updates, avoiding the direct involvement of adjacency features and thus improving computational efficiency. 
The update rules are governed by the following equation:
\begin{equation}
    \textstyle 
    \mathbf{X}^{(*)\prime}_\adj = \mathrm{FFN}\left(\mathbf{X}^{(*)}_\adj||\mathbf{X}^{(*)}\right), \;\;\;\;\mathbf{X}^{(*)\prime} = \mathrm{FFN}\left(\mathbf{X}^{(*)}_\adj||\mathbf{X}^{(*)}\right)
\end{equation}
Here, $(*)$ represents either the vertex set $\mathcal{V}$ or hyperedge set $\mathcal{E}$, and $||$ represents concatenation.

\subsection{Architecture Scaling}

Building upon a hybrid scaling strategy inspired by DeiT \cite{deit_paper} and ViG \cite{vig_paper}, HgVT achieves a balanced computational footprint across various model sizes. 
Table \ref{tab:scaling_variants} specifies transformer scaling hyperparameters and also delineates allocations for different vertex and edge types, where non-image vertices ($i\mathcal{V}$) are assigned fixed capacities as proposed by ViHGNN \cite{vihgnn_paper}. 
Additionally, we introduce the Ti-Lite variant (HgVT-Lt) aimed at facilitating ablations in a more computationally efficient manner within a constrained training budget.

\input{Figures/method/scaling_table}

To enhance efficiency, several potential paths exist to reduce parameters and FLOPS, aligned with the principles of graph neural networks. 
The feature matrices $\mathbf{X}^{(*)}$ and $\mathbf{X}^{(*)}_\adj$ can either be identical or have different dimensionalities,thereby simplifying the computational requirements of the FFN layers.
Additionally, tying both FFN layers to share weights further reduces the parameter count. 
Consistent with practices in Graph Attention Networks \cite{GAT_paper}, the weights for vertex self-attention ($W_Q,W_K,W_V$) and edge cross-attention ($W_K, W_V$) can also be tied. 
Implementing these strategies offers a range of options to tailor HgVT variants for balancing memory usage and computational efficiency, optimizing the model for various deployment environments based on performance needs.
